Can You Accept LaTeX Files from Strangers? Ten Years Later

It is well-known that Microsoft Word/Excel compatible documents or PDF files can contain malicious content. LaTeX files are unfortunately no exception either. LaTeX users often include third-party codes through sources or packages (.sty or .cls files). But those packages can execute malicious commands on the users' system, in order to capture sensitive information or to perform denial of service attacks. Checkoway et al. [3] were the first to warn LaTeX users of these threats. Collaborative cloud-based LaTeX editors and services compiling LaTeX sources are particularly concerned. In this paper, we have created a LaTeX package that collects system data and hides them inside the PDF file produced by the target. Then, we have measured what can be recovered by hackers using malicious LaTeX file on online services, and which measures those services have enforced to thwart the threats. Services defend themselves using sandbox or commands restrictions. Commands restrictions are more difficult to setup and we found one service (PMLatex) which is too permissive.

==> draft.tex <==




%\begin{table}[!ht]
%\begin{center}
%\begin{tabular}{p{2.1cm}|c|c|c|c}
%\textbf{Information} & \textbf{Overleaf} & \textbf{Papeeria} & \textbf{PLMlatex} & \textbf{CoCalc}  \\ %\hline
%User and group names & + & + & + & +   \\ \hline
%System & + & + & + & +   \\ \hline
%Hardware & - & - & - & -   \\ \hline
%CPU & + & + & - & +   \\ \hline
%Passwords & - & - & - & -  \\ \hline
%Outdated\newline software & + & + & - & +   \\ \hline
%Known\newline vulnerabilities & - & - & - & -   \\ \hline
%Open ports and\newline running services & - & - & - & +    \\ \hline
%Network\newline interfaces & - & - & + & -   \\ \hline
%Hostnames & - & + & + &  + \\ \hline
%Networking\newline protocols & - & + & + & +   \\ \hline
%Firewall\newline configurations & - & - & - &  -  \\ \hline
%Routing tables & - & - & - & +   \\ \hline
%Configuration of web servers & - & - & + & +   \\ \hline
%Web passwords & - & - & - & -   \\ \hline
%SSL certificates & - & - & - & - \\ 
%\end{tabular}
%\end{center}
%\caption{Information obtained}\label{tab:info}
%\end{table}

%\begin{table*}[!ht]
%\begin{center}%what if we split the table into 2 instead? yeah why not
%\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} %we can do that
%Service & \rotatebox[origin=c]{70}{\parbox{1.5cm}{\scriptsize User and\\ group names}} & \rotatebox[origin=c]{70}{\scriptsize System} & \rotatebox[origin=c]{70}{\scriptsize Hardware} & \rotatebox[origin=c]{70}{\scriptsize CPU} & \rotatebox[origin=c]{70}{\scriptsize Passwords} & \rotatebox[origin=c]{70}{\parbox{1cm}{\scriptsize Outdated software}} & \rotatebox[origin=c]{70}{\parbox{1.5cm}{\scriptsize Known\\ vulnerabilities}} & \rotatebox[origin=c]{70}{\parbox{1.8cm}{\scriptsize Open ports and\\ running services}} & \rotatebox[origin=c]{70}{\parbox{0.9cm}{\scriptsize Network\\ interfaces}} & \rotatebox[origin=c]{70}{\scriptsize Hostnames} & \rotatebox[origin=c]{70}{\parbox{1.2cm}{\scriptsize Networking\\ protocols}} & \rotatebox[origin=c]{70}{\parbox{1.2cm}{\scriptsize Firewall\\ configurations}} & \rotatebox[origin=c]{70}{\parbox{0.5cm}{\scriptsize Routing\\ tables}} & \rotatebox[origin=c]{70}{\parbox{1cm}{\scriptsize Server\\ configuration}} & \rotatebox[origin=c]{70}{\parbox{1cm}{\scriptsize Web\\ passwords}} & \rotatebox[origin=c]{70}{\parbox{1.5cm}{\scriptsize SSL certificates}} \\ \hline 
%Overleaf & \cmark{} & \cmark{} & \xmark{} & \cmark{} & \xmark{} & \cmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{}  \\ \hline
%Papeeria & \cmark{} & \cmark{} & \xmark{} & \cmark{} & \xmark{} & \cmark{} & \xmark{} & \xmark{} & \xmark{} & \cmark{} & \cmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{}\\ \hline
%PLMlatex & \cmark{} & \cmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \cmark{} & \cmark{} & \cmark{} & \xmark{} & \xmark{} & \cmark{} & \xmark{} & \xmark{} \\ \hline
%CoCalc & \cmark{} & \cmark{} & \xmark{} & \cmark{} & \xmark{} & \cmark{} & \xmark{} & \cmark{} & \xmark{} & \cmark{} & \cmark{} & \xmark{} & \cmark{} & \cmark{} & \xmark{} & \xmark{}\\
%\end{tabular}
%\end{center}
%\caption{Information obtained}\label{tab:info}
%\end{table*}

%\begin{tabular}{c|c|c|c|c|c|c|c|c} 
%Service & \rotatebox[origin=c]{70}{\parbox{0.9cm}{\scriptsize Network\\ interfaces}} & \rotatebox[origin=c]{70}{\scriptsize Hostnames} & \rotatebox[origin=c]{70}{\parbox{1.2cm}{\scriptsize Networking\\ protocols}} & \rotatebox[origin=c]{70}{\parbox{1.2cm}{\scriptsize Firewall\\ configurations}} & \rotatebox[origin=c]{70}{\parbox{0.5cm}{\scriptsize Routing\\ tables}} & \rotatebox[origin=c]{70}{\parbox{1cm}{\scriptsize Server\\ configuration}} & \rotatebox[origin=c]{70}{\parbox{1cm}{\scriptsize Web\\ passwords}} & \rotatebox[origin=c]{70}{\parbox{1.5cm}{\scriptsize SSL certificates}} \\ \hline 
%Overleaf & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} \\ \hline
%Papeeria & \xmark{} & \cmark{} & \cmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} \\ \hline
%PLMlatex & \cmark{} & \cmark{} & \cmark{} & \xmark{} & \xmark{} & \cmark{} & \xmark{} & \xmark{} \\ \hline
%CoCalc & \xmark{} & \cmark{} & \cmark{} & \xmark{} & \cmark{} & \cmark{} & \xmark{} & \xmark{} \\
%\end{tabular}
%hal

%can't read /proc/self/cgroup, not unix or can't read?
%DVI mode ???????

%plmtatex

%unix based
%can read files
%no docker? /proc/self/cgroup -> 2:name=systemd:/
%can read network interfaces :

%Configuration reseau; fichier gere par puppet plmbase::network
%auto lo iface lo inet loopback auto eth0 iface eth0 inet static address 172.16.101.70 netmask 255.255.255.0 post-up route add -net 172.16.0.0 netmask 255.255.0.0 gw 172.16.101.1 auto eth1 iface eth1 inet static address 147.210.130.30 netmask 255.255.255.128 gateway 147.210.130.126

%147.210.130.30 -> https://www.shodan.io/host/147.210.130.30

%hosts

%127.0.0.1 localhost  127.0.1.1 sharelatex.bordeaux sharelatex    The following lines are desirable for IPv6 capable hosts::1 ip6-localhost ip6-loopback  fe00::0 ip6-localnet  00::0 ip6-mcastprex  02::1 ip6-allnodes02::2 ip6-allrouter

%protocols

%Internet (IP) protocols     Updated from http://www.iana.org/assignments/protocol-numbers and othersources.    New protocols will be added on request if they have been ocially   assigned by IANA and are not historical.If you need a huge list of used numbers please install the nmap package.   ip 0 IP  internet protocol, pseudo protocol numberhopopt 0 HOPOPT  IPv6 Hop-by-Hop Option [RFC1883]  icmp 1 ICMP  internet control message protocoligmp 2 IGMP  Internet Group Management  ggp 3 GGP  gateway-gateway protocol1
%ipencap 4 IP-ENCAP  IP encapsulated in IP (ocially \IP")  st 5 ST  ST datagram modetcp 6 TCP  transmission control protocol  egp 8 EGP  exterior gateway protocoligp 9 IGP  any private interior gateway (Cisco)  pup 12 PUP  PARC universal packet protocoludp 17 UDP  user datagram protocol  hmp 20 HMP  host monitoring protocolxns-idp 22 XNS-IDP  Xerox NS IDP  rdp 27 RDP  "reliable datagram" protocoliso-tp4 29 ISO-TP4  ISO Transport Protocol class 4 [RFC905]  dccp 33 DCCP  Datagram Congestion Control Prot.  [RFC4340]xtp 36 XTP  Xpress Transfer Protocol  ddp 37 DDP  Datagram Delivery Protocolidpr-cmtp 38 IDPR-CMTP  IDPR Control Message Transport  ipv6 41 IPv6  Internet Protocol, version 6ipv6-route 43 IPv6-Route  Routing Header for IPv6  ipv6-frag 44 IPv6-Frag  Fragment Header for IPv6idrp 45 IDRP  Inter-Domain Routing Protocol  rsvp 46 RSVP  Reservation Protocolgre 47 GRE  General Routing Encapsulation  esp 50 IPSEC-ESP  Encap Security Payload [RFC2406]ah 51 IPSEC-AH  Authentication Header [RFC2402]  skip 57 SKIP  SKIP  ipv6-icmp 58 IPv6-ICMP  ICMP for IPv6ipv6-nonxt 59 IPv6-NoNxt  No Next Header for IPv6  ipv6-opts 60 IPv6-Opts  Destination Options for IPv6rspf 73 RSPF CPHB  Radio Shortest Path First (ocially CPHB)  vmtp 81 VMTP  Versatile Message Transporteigrp 88 EIGRP  Enhanced Interior Routing Protocol (Cisco)  ospf 89 OSPFIGP  Open Shortest Path First IGPax.25 93 AX.25  AX.25 frames  ipip 94 IPIP  IP-within-IP Encapsulation Protocoletherip 97 ETHERIP  Ethernet-within-IP Encapsulation [RFC3378]  encap 98 ENCAP  Yet Another IP encapsulation [RFC1241]99  any private encryption scheme  pim 103 PIM  Protocol Independent Multicastipcomp 108 IPCOMP  IP Payload Compression Protocol  vrrp 112 VRRP  Virtual Router Redundancy Protocol [RFC5798]l2tp 115 L2TP  Layer Two Tunneling Protocol [RFC2661]  isis 124 ISIS  IS-IS over IPv4sctp 132 SCTP  Stream Control Transmission Protocol  fc 133 FC  Fibre Channelmobility-header 135 Mobility-Header  Mobility Support for IPv6 [RFC3775]  udplite 136 UDPLite  UDP-Lite [RFC3828]mpls-in-ip 137 MPLS-in-IP  MPLS-in-IP [RFC4023]  manet 138  MANET Protocols [RFC5498]hip 139 HIP  Host Identity Protocol  shim6 140 Shim6  Shim6 Protocol [RFC5533]
%wesp 141 WESP  Wrapped Encapsulating Security Payload  rohc 142 ROHC  Robust Header Compression

%nginx.conf
%can't write

%user www-data; workerprocesses4;pid=run=nginx:pid;events  workerconnections768;multiaccepton;httpBasic Settingssendle on; tcpnopushon;tcpnodelayon;keepalivetimeout65;typeshashmaxsize2048;servertokensoff;1
%servernameshashbucketsize64;servernameinredirectoff;include /etc/nginx/mime.types; defaulttypeapplication=octetstream;Logging Settingsaccesslog=var=log=nginx=access:log;errorlog=var=log=nginx=error:log;Gzip Settingsgzip on; gzipdisable"msie6";gzipvaryon;gzipproxiedany;gzipcomplevel6;gzipbuffers168k;gziphttpversion1:1;gziptypestext=plaintext=cssapplication=jsonapplication=xjavascripttext=xmlapplication=xmlapplication=xml+rsstext=javascript;nginx-naxsi cong    Uncomment it if you installed nginx-naxsiinclude /etc/nginx/naxsicore:rules;nginx-passenger cong    Uncomment it if you installed nginx-passengerpassengerroot=usr;passengerruby=usr=bin=ruby;Virtual Host Configs
%include /etc/nginx/conf.d/*.conf; include /etc/nginx/sites-enabled/*;mail   See sample authentication script at:    http://wiki.nginx.org/ImapAuthenticateWithApachePhpScriptauthhttplocalhost=auth:php;pop3capabilities"T OP""USER";imapcapabilities"IMAP4rev1""UIDP LUS";

%papeeria 

%security mentioned in the ToS
%you are responsible for all content posted and activity that occurs under your account. 
%Do not violate the law and be nice to others
%distributing harmful or offensive content that is defamatory, obscene, abusive;
%violating the security or integrity of any computer, network or communications system;
%Scraping of public, non-personal information from Papeeria is allowed for research, archiving and indexing purposes. You may not scrape Papeeria for spamming purposes, including for the purposes of selling Papeeria users' personal information to anyone.

%CONTAINER INFO
%Most of the components involved into the Service operations run in isolated containers with the least possible privileges. In particular, any processing of user data which may include running arbitrary code happens inside a hardened container with its own file system, system resources usage limits and no network access.

%system commands enabled
%BUT 
%running with lualatex on tex live 2019 gives an error 
%=>
%! Undefined control sequence. 
%l.86 \initleak  Fatal error occurred,
%The control sequence at the end of the top line of your error message was never \def'ed. If you have misspelled it (e.g., `\hobx'), type `I' and the correct spelling (e.g., `I\hbox'). Otherwise just continue, and I'll forget about whatever was undefined.

%! TeX capacity exceeded, sorry [input stack size=5000].
%If you really absolutely need more capacity, you can ask a wizard to enlarge me.
%They also check the input size of the files and the output

%after moving back to tex-primitives we were able to run some commands
%DOCKER


%arxiv 
%users need to be endorsed before submitting their first paper

% Authorea does not support advanced LaTeX

%ARXIV
%Lua - failed  ! Emergency stop at \initleak -> \directlua
% stream version - pdfTeX error (ext5): cannot open file for embedding
% restricted \write18 enabled.


